Algorithms with Logarithmic or Sublinear Regret for Constrained Contextual Bandits

We study contextual bandits with budget and time constraints, referred to as constrained contextual bandits.The time and budget constraints significantly complicate the exploration and exploitation tradeoff because they introduce complex coupling among contexts over time.Such coupling effects make it difficult to obtain oracle solutions that assume known statistics of bandits. To gain insight, we first study unit-cost systems with known context distribution. When the expected rewards are known, we develop an approximation of the oracle, referred to Adaptive-Linear-Programming (ALP), which achieves near-optimality and only requires the ordering of expected rewards. With these highly desirable features, we then combine ALP with the upper-confidence-bound (UCB) method in the general case where the expected rewards are unknown {\it a priori}. We show that the proposed UCB-ALP algorithm achieves logarithmic regret except for certain boundary cases. Further, we design algorithms and obtain similar regret analysis results for more general systems with unknown context distribution and heterogeneous costs. To the best of our knowledge, this is the first work that shows how to achieve logarithmic regret in constrained contextual bandits. Moreover, this work also sheds light on the study of computationally efficient algorithms for general constrained contextual bandits.

==> abstract_submitted.tex <==
We study contextual bandits with budget and time constraints under discrete contexts, referred to as constrained contextual bandits. The budget and time constraints significantly increase the complexity of exploration-exploitation tradeoff because they introduce coupling among contexts. Such coupling effects make it difficult to obtain oracle solutions that assume known statistics of bandits. To gain insight, we first study unit-cost systems, where the costs of all actions under any context are identical. We  develop near-optimal approximations of the oracle, which are then combined with upper confidence bound (UCB) method in the general case where the expected rewards are unknown a priori. We show that our proposed algorithms, named UCB-PB and UCB-ALP, achieve logarithmic regret except in certain boundary cases. Last, we discuss the extension of the proposed algorithms into general-cost systems. To the best of our knowledge, the proposed algorithms are the first easily-implementable algorithms to achieve sublinear regret in constrained contextual bandits. 

==> app_bound_of_occurances.tex <==



==> app_oracle_twocontext.tex <==
%%%%%%%%%%
\section{Proof of Corollary 1: Oracle algorithm for Two-Context Systems}\label{app:proof_opt_two_context}
%%%%%%%%%%
It is obvious that $j_{\rm th}(\tau, b) = 1$  for $b\geq \tau$ and we only need to show that $j_{\rm th}(\tau, b) = 2$ for $b < \tau$.
To show $j_{\rm th}(\tau, b) = 2$, it suffices to show that the optimal threshold for $b = \tau -1$ is $j_{\rm th}(\tau, b) = 2$,
which can be proved by induction as follows.

When $\tau = 2$, $b = 1$, it is optimal to take the best action when $X_{T-\tau + 1} = 2$, and the value function is
\begin{eqnarray}
V_2(1) = \pi_2 u_2^* + \pi_1(\pi_1 u_1^* + \pi_2 u_2^*).
\end{eqnarray}

Assume that $j_{\rm th}(b', \tau') = 2$ is true for all $2 \leq \tau' \leq \tau$ and $b' = \tau' - 1$.
Then the value function can be calculated in a recursive manner as follows:
\begin{eqnarray}
&& V_{\tau-1}(b-1) \nonumber \\
&=&  \pi_2[u_2^* + V_{\tau-2}(b-2)] + \pi_1 (b-1)(\pi_1 u_1^* + \pi_2 u_2^*),\nonumber\\
&& V_{\tau-2}(b-2) \nonumber \\
&=&  \pi_2[u_2^* + V_{\tau-3}(b-3)] + \pi_1 (b-2)(\pi_1 u_1^* + \pi_2 u_2^*),\nonumber\\
&&\ldots \ldots \nonumber\\
&&V_2(1)  \pi_2 u_2^* + \pi_1(\pi_1 u_1^* + \pi_2 u_2^*),\nonumber
\end{eqnarray}
implying that
\begin{eqnarray}
&&V_{\tau-1}(b-1) \nonumber \\
&=&  \frac{\pi_2 u_2^*(1 - \pi_2^{b-1}) + (\pi_1 u_1^* + \pi_2 u_2^*)(b-1 -b\pi_2 + \pi_2^b)}{1 - \pi_2}. \nonumber
\end{eqnarray}
On the other hand, since $b = \tau -1$,
\begin{eqnarray}
V_{\tau-1}(b) = b(\pi_1 u_1^* + \pi_2 u_2^*).
\end{eqnarray}
Thus,
\begin{eqnarray}
&&{V_{\tau-1}(b) - V_{\tau-1}(b-1)} \nonumber \\
&=&  b(\pi_1 u_1^* + \pi_2 u_2^*) \nonumber \\
&&- \frac{\pi_2 u_2^*(1 - \pi_2^{b-1})   + (\pi_1 u_1^* + \pi_2 u_2^*)(b-1 -b\pi_2 + \pi_2^b)}{1 - \pi_2}\nonumber \\
&= &{ u_1^* + \pi_2^b(u_2^* - u_1^*) > u_1^*.}
\end{eqnarray}
Consequently, the optimal threshold  is $j_{\rm th}(\tau, b) = 2$ for all $\tau$ and $b = \tau -1$. According to Theorem~\ref{thm:opt_threshold_struct} and the definition of threshold, we know that $j_{\rm th}(\tau, b) = 2$  for all  cases with
$b < \tau$.

==> app_regret_newproof.tex <==
\newpage
\begin{theorem}\label{thm:regret_ucb_alp_new}
Given $\pi_j$'s, $u_{j,k}$'s and a fixed $\rho \in [0,1]$, the regret of UCB-ALP satisfies:\\
1) (Non-boundary cases) if $\rho \neq q_j$, $1 \leq j \leq J-1$, then the regret of UCB-ALP is $R_{\rm{UCB-ALP}}(T, B) = O\big(JK\log T\big)$.\\
%\begin{eqnarray}
%\limsup_{T\to \infty} \frac{R_{\rm{UCB-ALP}}(T, B)}{\log T} \leq \Theta^{\rm (c)}_{\rm nb} + \Theta^{\rm (a)}, \nonumber
%\end{eqnarray}
%where $\Theta^{\rm (c)}_{\rm nb} = [\bar{u}^* + v(\rho)]\bigg\{\sum_{j = 1}^{\tilde{j}(\rho)}\sum_{k=1}^K\frac{27}{2g_{\tilde{j}(\rho)+1} [\Delta^{(j)}_{\tilde{j}(\rho)+1,k}]^2}
%+ \sum_{j =\tilde{j}(\rho)+2}^{J}\sum_{k=1}^K\frac{27}{2g_j [\Delta^{(\tilde{j}(\rho)+1)}_{j,k}]^2} + KJ \bigg\}$,
%$\Theta^{\rm (a)} = \sum_{j=1}^J \sum_{k \neq k_j^*} \big(\frac{2}{\Delta_{j,k}^{(j)}} + 2\Delta_{j,k}^{(j)}\big)$
%with $\bar{u}^* = \sum_{j = 1}^J \pi_j u_j^*$, and $v(\rho)$ defined in \eqref{eq:LP_single_step_value}.\\
2) (Boundary cases) if $\rho = q_j$ for some $j \in \{ 1,2, \ldots, J-1\}$, then the regret of UCB-ALP is $R_{\rm{UCB-ALP}}(T, B) = O\big(\sqrt{T} + JK\log T \big)$.
%\begin{eqnarray}
%R_{\text{UCB-ALP}}(T, B) \leq \Theta^{\rm (o)} \sqrt{T}  + [\Theta^{\rm (c)}_{\rm b} + \Theta^{\rm (a)}]\log T + O(1), \nonumber
%\end{eqnarray}
%where $\Theta^{\rm (o)} =  2(u_1^* - u_J^*) \sqrt{\rho (1-\rho)}$,
%%$\Theta^{\rm (a)}$ is defined as in Theorem~\ref{thm:regret_ucb_alp_nonboundary},
%\begin{align}
%\Theta^{\rm (c)}_{\rm b} = [\bar{u}^* + v(\rho)]\bigg\{\sum_{j = 1}^{\tilde{j}(\rho)-1}\sum_{k=1}^K\frac{27}{2g'_{\tilde{j}(\rho)} [\Delta^{(j)}_{\tilde{j}(\rho),k}]^2}
%+ \sum_{j =\tilde{j}(\rho)+1}^{J}\sum_{k=1}^K\frac{27}{2g'_j [\Delta^{(\tilde{j}(\rho))}_{j,k}]^2} + KJ \bigg\},
%\end{align}
%and $g'_j = \min\big\{\pi_j, \frac{1}{2}(\rho - q_{\tilde{j}(\rho)-1}), \frac{1}{2}(q_{\tilde{j}(\rho)+1} -\rho)\big\}$.
\end{theorem}


\begin{proof}
We bound the regret of UCB-ALP by comparing its performance  with the benchmark $\widehat{U}(T,B)$. To obtain this upper bound, we first partition the regret according to the sources and then bound the each part of regret, respectively.

Before presenting the proof, we first introduce a notation that will be widely used later. For contexts $j$ and $j'$, and an action $k$, let $\Delta_{j,k}^{(j')}$ be the difference between the expected reward for action $k$ under context $j$ and the highest expected reward under context $j'$, i.e., $\Delta_{j,k}^{(j')} = u_{j'}^* - u_{j,k}$.
When $j' = j$, $\Delta_{j,k}^{(j)}$ is the difference of expected reward between the suboptimal action $k$ and the best action under context $j$.


%%%%%%%%%%
\subsection{Step 1: Partition the Regret}
%%%%%%%%%%

Note that the total reward of the oracle solution $U^*(T,B)  \leq \widehat{U}(T,B)$. Thus, we can bound the regret of UCB-ALP by comparing its total expected reward $U_{\rm UCB-ALP}(T,B)$ with $\widehat{U}(T,B)$, i.e.,
\begin{eqnarray}
&&R_{\rm {UCB-ALP}}(T, B) \nonumber \\
&=& U^*(T,B) - U_{\rm UCB-ALP}(T,B) \nonumber \\
& \leq &\widehat{U}(T,B) - U_{\rm UCB-ALP}(T,B) \nonumber\\
&= & T v(\rho) - \sum_{j = 1}^J \sum_{k =1}^K u_{j,k} \mathbb{E}[C_{j,k}(T)].
\end{eqnarray}
The total expected reward of UCB-ALP can be further divided as
\begin{eqnarray}
&& U_{\rm UCB-ALP}(T,B) \nonumber \\
& =&  \sum_{j = 1}^J u_j^* \mathbb{E}\big[\sum_{k=1}^K C_{j,k}(T)\big] - \sum_{j=1}^J \sum_{k=1}^K \Delta_{j,k}^{(j)}\mathbb{E}[C_{j,k}(T)] \nonumber \\
& =&  \sum_{j = 1}^J u_j^*\mathbb{E}\big[C_{j}(T)\big] - \sum_{j=1}^J \sum_{k=1}^K \Delta_{j,k}^{(j)}\mathbb{E}[C_{j,k}(T)], \nonumber
\end{eqnarray}
where $C_j(T) = \sum_{k=1}^K C_{j,k}(T)$ is the total number that actions have been taken under context $j$ up to round $T$.

Consequently, the regret of UCB-ALP can be bounded as
\begin{eqnarray}\label{eq:regret_ucb_alp__nonboundary_details}
R_{\rm {UCB-ALP}}(T, B) \leq R_{\rm {UCB-ALP}}^{({\rm a})}(T, B) + R_{\rm {UCB-ALP}}^{({\rm c})}(T, B),
\end{eqnarray}
where
\begin{eqnarray}
R_{\rm {UCB-ALP}}^{({\rm a})}(T, B) = \sum_{j=1}^J \sum_{k=1}^K \Delta_{j,k}^{(j)}\mathbb{E}[C_{j,k}(T)], \nonumber
\end{eqnarray}
and
\begin{eqnarray}
R_{\rm {UCB-ALP}}^{({\rm c})}(T, B) = T v(\rho) - \sum_{j  = 1}^J u_j^*\mathbb{E}[C_j(T)]. \nonumber
\end{eqnarray}

Eq.~\eqref{eq:regret_ucb_alp__nonboundary_details} clearly shows that the regret of the UCB-ALP algorithm can be divided into two parts: the first part $R_{\rm {UCB-ALP}}^{({\rm a})}(T, B)$ is from taking  suboptimal actions under a given context; the second part $R_{\rm {UCB-ALP}}^{({\rm c})}(T, B)$ is from the deviation of remaining budget $b_{\tau}$ and context ranking errors.

%%%%%%%%%%
\subsection{Step 2: Bound Each Part of Regret}
%%%%%%%%%%

\subsubsection{Step 2.1: Bound of $R_{\text{UCB-ALP}}^{\rm (a)}(T, B)$.}
For the regret from action ranking errors,
we show in Lemma~\ref{thm:regret_withincontext} that $R_{\text{UCB-ALP}}^{\rm (a)}(T, B) = O(\log T)$ using similar techniques for traditional UCB methods \cite{Golovin2009Lecture}.
\begin{lemma}\label{thm:regret_withincontext}
Under UCB-ALP, the regret due to the action ranking errors within context $j$ satisfies
\begin{eqnarray} \label{eq:regret_ucb_alp_regret_withincontext}
R_{\text{UCB-PB}}^{\rm (a)}(T, B) \leq \sum_{j=1}^J \sum_{k \neq k_j^*} \bigg[\big(\frac{2}{\Delta_{j,k}^{(j)}} + 2\Delta_{j,k}^{(j)}\big) \log T + 2 \Delta_{j,k}^{(j)}\bigg].
\end{eqnarray}
\end{lemma}
\begin{proof}
For $k \neq k_j^*$, let $\ell_{j,k}^{(j)} = \frac{2\log T}{(\Delta_{j, k}^{(j)})^2}$. According to Lemma~\ref{thm:context_action_pair_errorprob}, we have
\begin{eqnarray}
&& \mathbb{E}[C_{j,k}(T)] \nonumber \\
&\leq& \ell_{j,k}^{(j)} + \sum_{t = 1}^T \mathbb{P}\{X_t = j, A_t = k, C_{j,k}(t-1) \geq \ell_{j,k}^{(j)}\} \nonumber \\
&\leq & \ell_{j,k}^{(j)} + \sum_{t = 1}^T \mathbb{P}\{X_t = j, A_t = k | C_{j,k}(t-1) \geq \ell_{j,k}^{(j)}\} \nonumber \\
&\leq & \ell_{j,k}^{(j)} + 2\sum_{t = 1}^Tt^{-1}. \nonumber
\end{eqnarray}
The conclusion then follows by the facts that $\sum_{t = 1}^T t^{-1} \leq 1 + \log T$ and $R_{\text{UCB-ALP}}^{\rm (a)}(T, B) =  \sum_{j = 1}^J\sum_{k \neq k_j^*} \Delta_{j,k}^{(j)} \mathbb{E}[C_{j,k}(T)]$.
\end{proof}

\subsubsection{Step 2.2: Bound of $R_{\text{UCB-ALP}}^{\rm (c)}(T, B)$.}
Next, we show that the second part $R_{\rm {UCB-ALP}}^{({\rm c})}(T, B)$ is also in the order of $O(\log T)$.
We mainly focus on the proof for the non-boundary cases, and discuss the boundary cases later.

From Algorithm~\ref{alg:ucb_alp}, we can see that the evolution of the remaining budget also affects the execution of the UCB-ALP algorithm. Under the assumption of known context distribution, it can be verified that Lemma~\ref{thm:alp_to_hypergeo} holds under UCB-ALP, i.e., the remaining budget $b_{\tau}$ follows the hypergeometric distribution and has the properties described in Lemma~\ref{thm:alp_to_hypergeo}. We define an event $\mathcal{E}_{\rm budget, 0}(t)$ as follows,
\begin{eqnarray}
\mathcal{E}_{\rm budget, 0}(t)  = \{(\rho - \delta) \tau \leq b_{\tau} \leq (\rho + \delta) \tau\}, \nonumber
\end{eqnarray}
where $\delta$ is given by
\begin{eqnarray}
\delta = \frac{1}{2}\min\{\rho - q_{\tilde{j}(\rho)}, q_{\tilde{j}(\rho)+1} -\rho\}. \nonumber
\end{eqnarray}
According to Lemma~\ref{thm:alp_to_hypergeo}, we have
\begin{eqnarray}
\mathbb{P}\{\urcorner\mathcal{E}_{\rm budget, 0}(t)\}
= \mathbb{P}\{ b_{\tau} <  (\rho -\delta) \tau\} + \mathbb{P}\{ b_{\tau} >  (\rho +\delta) \tau\} \leq 2e^{-2\delta^2 (T-t + 1)}. \nonumber
\end{eqnarray}

Now we analyze $\mathbb{E}[C_j(T)]$ under UCB-ALP. We first show the upper bound on $\mathbb{E}[C_j(T)]$ for $j \geq \tilde{j}(\rho) + 1$. Then, using the fact of $\sum_{j = 1}^J C_j(T) = B$, we can obtain the lower bound on $\mathbb{E}[C_j(T)]$ for $j \leq \tilde{j}(\rho) + 1$ and the upper bound of $R_{\text{UCB-ALP}}^{\rm (c)}(T, B)$.

For $j > \tilde{j}(\rho) + 1$ and $1 \leq k \leq K$, let $\ell_{j,k}^{(\tilde{j}(\rho)+1)} = \frac{2 \log T}{[\Delta_{j,k}^{(\tilde{j}(\rho)+1)}]^2}$. We know that if $(\rho - \delta) \tau \leq b_{\tau} \leq (\rho + \delta) \tau$, context $j$ can only be played when there exists a $j' \leq \tilde{j}(\rho)+1$ such that $\hat{u}_j(t) \geq \hat{u}_{j'}(t)$. Then, with a slight modification to the analysis of Lemma~\ref{thm:regret_withincontext}, we have
\begin{eqnarray}
\mathbb{E}[C_{j,k}(T)] &\leq& \ell_{j,k}^{(\tilde{j}(\rho)+1)} + \sum_{t = 1}^T \mathbb{P}\{X_t = j, \exists wrong-rank, C_{j,k}(t-1) \geq \ell_{j,k}^{(\tilde{j}(\rho)+1)}, \mathcal{E}_{\rm budget, 0}(t)\} + \sum_{t = 1}^T \mathbb{P}\{\urcorner\mathcal{E}_{\rm budget, 0}(t)\} \nonumber \\
&\leq&\ell_{j,k}^{(\tilde{j}(\rho)+1)} + 2(1 + \log T) + \frac{2e^{-2\delta^2}}{1 - e^{-2\delta^2}}, \nonumber
\end{eqnarray}
implying that
\begin{eqnarray} \label{eq:ub_supoptimal_context}
\mathbb{E}[C_j(T)] \leq \sum_{k=1}^K \ell_{j,k}^{(\tilde{j}(\rho)+1)} + 2K\big(1 + \log T + \frac{2e^{-2\delta^2}}{1 - e^{-2\delta^2}}\big).
\end{eqnarray}


For $j = \tilde{j}(\rho) + 1$, we have
\begin{eqnarray}
\mathbb{E}[C_{j,k}(T)] &\leq& \ell_{\tilde{j}(\rho)+1,k}^{(j)} + \sum_{t = 1}^T \mathbb{P}\{X_t = j, \exists wrong-rank, C_{j,k}(t-1) \geq \ell_{j,k}^{(\tilde{j}(\rho)+1)}, \mathcal{E}_{\rm budget, 0}(t)\} \nonumber \\
&& + \sum_{t = 1}^T \mathbb{P}\{X_t = j, no wrong-rank, C_{j,k}(t-1) \geq \ell_{j,k}^{(\tilde{j}(\rho)+1)}, \mathcal{E}_{\rm budget, 0}(t)\} + \sum_{t = 1}^T \mathbb{P}\{\urcorner\mathcal{E}_{\rm budget, 0}(t)\} \nonumber \\
&\leq&\ell_{\tilde{j}(\rho)+1,k}^{(j)} + 2(1 + \log T)  + \frac{2e^{-2\delta^2}}{1 - e^{-2\delta^2}}, \nonumber
\end{eqnarray}





\end{proof} 

\section{General UCB-ALP}

How to show its logarithmic regret?

Analyze the scenarios where a certain context-action pair can be pulled:

1) $\hat{u}_{j,k}/c_{j,k}$ is large;

2) $(\hat{u}_{j,k_1} - \hat{u}_{j,k_2})/(c_{j, k_1} - c_{j, k_2})$ is larger, then $\hat{u}_{j,k_1}$ will be pulled. Moreover, it will be greater than 0 with high probability $O(1/T)$ if $(j,k_1)$ has been pulled for sufficient times.
\begin{lemma} \label{thm:hetcost_ucb_rank}
1) If $u_{j_1,k_1}/c_{j_1,k_1} <  u_{j_2,k_2}/c_{j_2,k_2}$, then $\mathbb{P}\{\hat{u}_{j_1,k_1}(t)/c_{j_1,k_1} \geq   \hat{u}_{j_2,k_2}(t)/c_{j_2,k_2}| C_{j_1, k_1}(t-1) \geq ?? \} \leq t^{-1}$.

2) For contexts $j_1$, $j_2$, and actions $k_{11}$, $k_{12}$, $k_{21}$, and $k_{22}$, if $u_{j_1,k_{11}} > u_{j_1,k_{12}}$, $u_{j_2,k_{21}} > u_{j_2,k_{22}}$, and $\frac{u_{j_1,k_{11}} - u_{j_1,k_{12}}}{c_{j_1,k_{11}} - c_{j_1,k_{12}}} <  \frac{u_{j_2,k_{21}} - u_{j_2,k_{22}}}{c_{j_2,k_{21}} - c_{j_2,k_{22}}}$, then
\begin{equation}
\mathbb{P}\big\{ \frac{u_{j_1,k_{11}}(t) - u_{j_1,k_{12}}(t)}{c_{j_1,k_{11}} - c_{j_1,k_{12}}} \geq  \frac{u_{j_2,k_{21}}(t) - u_{j_2,k_{22}}(t)}{c_{j_2,k_{21}} - c_{j_2,k_{22}}} \big| C_{j_1, k_{11}}(t-1) \geq \red{TBD} ?? , C_{j_2, k_{22}}(t-1) \geq  \red{TBD}\big\} \leq \frac{1}{t}.
\end{equation}
\end{lemma}

\textbf{The maxim of ``Optimism in the Face of Uncertainty''}: being optimistic within the confidence range; if one context-action should not be pulled that much, it will be finally identified (as soon as it has been pulled sufficiently)!

\textbf{The key idea of proof:} a context-action pair $(j,k)$ could only be pulled when it has large UCB. If it has been pulled for enough times, its UCB will be relatively accurate and will not be over pulled.

According to Lemma~\ref{thm:hetcost_ucb_rank}, we know that there exists a positive number $\delta_u$ such that if $|\hat{u}_{j,k}(t) - u_{j,k}| \leq \delta_u$, then the UCB-ALP will provide a correct rank (and thus \blue{a plausible solution}). 

Furthermore, we only need to consider the cases where there will actually result in regret and only consider  the context-action pairs with positive probability.
Let $\hat{C}_{j,k}(t)$ be the number of slots where $\hat{p}_{j,k}(t') > \delta_p > 0$, but $|\hat{u}_{j,k}(t') - u_{j,k}| \geq \delta_u$ up to $t$, i.e.,
\begin{equation}
\hat{C}_{j,k}(t) = \sum_{t' = 1}^{t}\mathbbm{1}(\hat{p}_{j,k}(t') > \delta_p, |\hat{u}_{j,k}(t') - u_{j,k}| \geq \delta_u).
\end{equation}
Then we can bound $\hat{C}_{j,k}(t)$ as $\hat{C}_{j,k}(t)  = O(\log T)$. 

Note that a suboptimal solution will be implemented only when there exists a context-action pair $(j,k)$ such that $\hat{p}_{j,k}(t') > \delta_p > 0$ and $|\hat{u}_{j,k}(t') - u_{j,k}| \geq \delta_u$. Summarize over all context-actions pairs, we know that the total regret will be bounded as $O(\log T)$. 


==> app_threshold_struct.tex <==
%%%%%%%%%%
\section{Proof of Theorem 1: Threshold Structure of DP}\label{app:proof_opt_threshold_struct}
%%%%%%%%%%
Recall that the dynamic programming (DP) value function $V_{\tau}(b)$ is the maximum expected total rewards when the remaining time is $\tau$ and remaining budget is $b$. As discussed in Section~\ref{sec:oracle_solution}, the value function can be expressed as follows:
%\begin{eqnarray}
%V_{\tau}(b) =
%\begin{cases}
%0,  &\text{if $\tau = 0$}, \\
%\mathbb{E}_{X_{T - \tau+1}}\big\{\max_{\nu \in \{0, 1\land b\}} [\nu u_{X_{T - \tau+1}}^* + V_{\tau-1}(b - \nu)] \big\}, &\text{otherwise},
%\end{cases}
%\end{eqnarray}
\begin{eqnarray}
V_{\tau}(b) = 0,  \text{if $\tau = 0$}, \nonumber \\
\end{eqnarray}
and otherwise,
\begin{eqnarray}
V_{\tau}(b) =
\mathbb{E}_{X_{T - \tau+1}}\big\{\max_{\nu \in \{0, 1\land b\}} [\nu u_{X_{T - \tau+1}}^* + V_{\tau-1}(b - \nu)] \big\}, \nonumber
\end{eqnarray}
where $1 \land b = \min\{1,b\}$. We show the optimality of the threshold algorithm by investigating the properties of the value function.

When $b > 0$, $\tau > 0$, and $X_{T- \tau+1} = j$, an optimal algorithm would choose an action $\nu \in \{0, 1\}$ that maximizes $\nu u_{X_{T - \tau+1}}^* + V_{\tau-1}(b - \nu)$, i.e.,
\begin{eqnarray}
V_{\tau -1}(b) \underset{\nu = 1}{\overset{\nu = 0}{\gtrless}} u_j^* + V_{\tau-1}(b - 1).
\end{eqnarray}
The above criterion can be rewritten as
\begin{eqnarray}
V_{\tau-1}(b) - V_{\tau-1}(b - 1)\underset{\nu = 1}{\overset{\nu = 0}{\gtrless}} u_j^*.
\end{eqnarray}
This implies that if $\nu = 1$ for context $j$, then $\nu = 1$ for all $j' > j$.

On the other hand, for given $j$, if $V_{\tau-1}(b+1) - V_{\tau-1}(b) \leq V_{\tau-1}(b) - V_{\tau-1}(b - 1)$, i.e., $V_{\tau-1}(b+1) + V_{\tau-1}(b - 1) \leq 2V_{\tau-1}(b)$, then  $\nu = 1$ for remaining budget $b$ implies $\nu = 1$ for all $b' > b$. Namely, the concavity of the value function on $\mathbb{N}$ is a sufficient condition for the optimality of the threshold algorithm. We can show the concavity of $V_{\tau}(b)$ by induction to $\tau$.

When $\tau = 0$,
$V_0(b)$ is concave on $\mathbb{N}$ since $V_0 (b) = 0$ for all $b \in \mathbb{N}$. For $\tau > 0$, assume $V_{\tau-1}(b)$ is a concave function on $\mathbb{N}$. Let $V_{\tau,j}(b)$ be the value function conditioned on $X_{T-\tau+1} = j$, i.e.,
\begin{eqnarray}
V_{\tau,j}(b) &=& \max_{\nu \in \{0, 1\land b\}} [\nu u_j^* + V_{\tau-1}(b - \nu)].
\end{eqnarray}
We note that when $b \geq 1$, $V_{\tau,j}(b) = \max_{\nu \in \{0, 1\}} [\nu u_j^* + V_{\tau-1}(b - \nu)]$ is concave since the maximization operation preserves concavity. To extend the concavity to the entire set of $\mathbb{N}$, it suffices to show that
\begin{eqnarray}\label{eq:grad_1}
V_{\tau,j}(0) + V_{\tau,j}(2) \leq 2V_{\tau,j}(1).
\end{eqnarray}
Note that
\begin{eqnarray}
V_{\tau,j}(0) &=& 0, \nonumber \\
V_{\tau,j}(2) &=& \max\{V_{\tau-1}(2), u_j^* + V_{\tau-1}(1)\}, \nonumber\\
2V_{\tau,j}(1) & = & \max\{2V_{\tau-1}(1), 2u_j^*  \} \nonumber.
\end{eqnarray}
Further, $u_j^* + V_{\tau-1}(1) \leq \max\{2V_{\tau-1}(1), 2u_j^*  \}$, and $V_{\tau-1}(2) = V_{\tau-1}(2) + V_{\tau-1}(0)\leq 2V_{\tau-1}(1)$ (because the concavity of $V_{\tau-1}(b)$ on $\mathbb{N}$). Thus, inequality~\eqref{eq:grad_1} holds and $V_{\tau,j}(b)$ is concave on $\mathbb{N}$, and $V_{\tau}(b) = \mathbb{E}_{X_{T-\tau+1}}V_{\tau,X_{T-\tau+1}}(b)$ is concave on  $\mathbb{N}$ because the expectation operation preserves concavity.

Consequently, $V_{\tau}(b)$ is concave on $\mathbb{N}$ for all $1 \leq \tau \leq T$, and the threshold algorithm is optimal.


==> het_cost.tex <==
\section{Extensions} \label{sec:exten}


\subsection{Constrained Contextual Bandits with Unknown Context Distributions} \label{subsec:unknown_dist}



\subsection{Constrained Contextual Bandits with Heterogeneous Costs} \label{subsec:het_cost}
{In this section, we discuss how to use the insight from unit-cost systems for the design of algorithms in heterogeneous-cost systems where cost $c_{j,k}$ depends on $j$ and $k$.
We only discuss the main results here due to space limitations. Details can be found in Appendix~\ref{app:het_cost} in the supplementary material.}

{When the statistics of bandits are known to the agent, the ALP algorithm can be generalized to heterogeneous-cost systems. With heterogeneous costs, the quality of an action $k$ under a context $j$ is roughly captured by its \emph{normalized expected reward}, defined as $\eta_{j,k} = u_{j,k}/c_{j,k}$. However, the agent cannot only focus on the ``best'' action, i.e., $k_j^* = \argmax_{k \in \mathcal{A}} \eta_{j,k}$, for context $j$.
This is because there may exist another action $k'$ such that $\eta_{j,k'} < \eta_{j,k_{j}^*}$, but $u_{j,k'} > u_{j,k_j^*}$ (and of course, $c_{j,k'} > c_{j, k_j^*}$). If the budget  allocated to context $j$ is sufficient, then the agent may take action $k'$ to maximize the expected reward. Therefore, the ALP algorithm in this case needs to decide the probability to take action $k$ under context $j$, by solving an LP problem with an additional constraint that only one action can be taken under each context.
%Unlike unit-cost systems, the remaining budget $b_{\tau}$ does not follow any classic distribution in heterogeneous-cost systems. However, we can show that its expectation $\mathbb{E}[b_{\tau}] = \rho \tau$. Moreover, the concentration property still holds in this general case by the method of averaged bounded differences \cite{Dubhashi2009Concentration}.
We can show that  ALP achieves $O(1)$ regret in non-boundary cases, and $O(\sqrt{T})$ regret in boundary cases.
We note that the regret analysis of ALP in this case is much more difficult due to the additional constraint that couples all actions under each context. }

{When the expected rewards are unknown, it is difficult in general to combine ALP with the UCB method since the ALP algorithm in this case not only requires the ordering of $\eta_{j,k}$'s, but also the ordering of $u_{j,k}$'s and the ratios $\frac{u_{j,k_1} - u_{j, k_2}}{c_{j,k_1} - c_{j, k_2}}$. As a special case, when all actions have the same cost under a given context, i.e., $c_{j,k} = c_j$ for all $k$ and $j$, the UCB-ALP can be extended  by defining the UCBs for the normalized expected rewards $\eta_{j,k}$ with appropriate scaling such that $Y_{k,t}/c_j \in [0,1]$ if $X_t = j$. However, it is still an open problem to design algorithms for general heterogeneous-cost systems.}

%Therefore, we consider an LP problem $\mathcal{LP}'_{T,B}$, where the decision variable $p_{j,k}$ is the probability that action $k$ is taken under context $j$.
%We construct an LP problem $\mathcal{LP}'_{T,B}$, which is similar to $\mathcal{LP}_{T,B}$ but take all actions into account under each context. Since the agent can only take at most one action under each context, additional constraints $\sum_{k = 1}^K p_{j,k} \leq 1$, $1 \leq j \leq J$, appear in $\mathcal{LP}'_{T,B}$. With these constraints, obtaining explicit representations for the solution of $\mathcal{LP}'_{T,B}$ is difficult. By analyzing the structure of the problem $\mathcal{LP}'_{T,B}$, we can eliminate certain actions under each contexts without affecting the optimal solution of $\mathcal{LP}'_{T,B}$. We define the set of remaining actions as the candidate set for each context and propose an algorithm for finding the candidate sets. Then, we obtain the explicit presentation of the solution, which also following a threshold structure,  by relaxing the probability constraints with a transformation. The ALP algorithm in this case uses the solution of $\mathcal{LP}'_{\tau,b}$ when the remaining time is $\tau$ and the remaining budget is $b$, and can be shown to achieve similar performance as unit-cost systems.






